On the overlooked issue of defining explanation objectives for local-surrogate explainers

Local surrogate approaches for explaining machine learning model predictions have appealing properties, such as being model-agnostic and flexible in their modelling. Several methods exist that fit this description and share this goal. However, despite their shared overall procedure, they set out different objectives, extract different information from the black-box, and consequently produce diverse explanations, that are -- in general -- incomparable. In this work we review the similarities and differences amongst multiple methods, with a particular focus on what information they extract from the model, as this has large impact on the output: the explanation. We discuss the implications of the lack of agreement, and clarity, amongst the methods' objectives on the research and practice of explainability.

==> sections/shapley.tex <==
\section{Shapley Values}
\todo[inline]{not finished}
Shapley Values originate in cooperative game theory and provide a way of splitting a value amongst a coalition of players [reference]. They are the unique solution that satisfies constraints:
\begin{enumerate}
    \item a
    \item b
    \item c
\end{enumerate}
These have been adapted to machine learning by ... .

[notations]

The Shapley Value for feature (/player) $i$ for the prediction of instance (/game) $x$ is defined as:
\begin{equation}
\varphi_{i}(x)=\sum_{Q \subseteq S \backslash\{i\}} \frac{|Q| !(|S|-|Q|-1) !}{|S| !}\left(\Delta_{Q \cup\{i\}}(x)-\Delta_{Q}(x)\right)
\label{eq:example_shapley_value}
\end{equation}

$\Delta_{Q}(x)$ denotes the value of the game when the coalition is formed by players in set $Q$ only. In our case our objective is to assign feature importance measures to a set of features for a prediction of a given fixed black-box model. Therefore, inputs can only be of size $|S|$. The function used in [references] instead is:

\begin{equation}
    \Delta_{Q}(x) = \mathbb{E}[f(X)~|~X_i=x_i, \forall i \in Q] = \mathbb{E}_{p(X_{\neg Q}|X_Q)}[f(X)]
    \label{eq:example_delta_shapley}
\end{equation}

\paragraph{Approximation 1.:} Shapley Values obtained are not with respect to $f$, but with respect to expectations over $f$ instead.

Unless $f$ is of specific nature (e.g. linear model, tree-base model) then computing integrals of the form of Eq.\ref{eq:example_delta_shapley} -necessary for computing Eq.\ref{eq:example_shapley_value}- can be intractable. [In our case we are dealing with black-box models assuming the model is complex and therefore computing Eq.\ref{eq:example_delta_shapley} can only be done in approximation.]

In [kononenko] the approximation is of the form ...

In SHAP \cite{Lundberg_Lee_2017} the Shapley Values are estimated using\footnote{This is the solution of the problem formulated in Theorem 2 of \cite{Lundberg_Lee_2017}.}:

\begin{equation}
\label{eq:kshap_regression}
\phi=\left(X^{T} W X\right)^{-1} X^{T} W y
\end{equation}
where $X \in \mathbb{R}^{2^M\times M}$ is the matrix of all binary vectors of size $M$, $W$ is a diagonal matrix with values corresponding to the Shapley Kernel evaluated on every row of $X$. Every element of $y$ corresponds to one evaluation of $\Delta_{Q}(x)$ (See Eq.\ref{eq:example_delta_shapley}) for all sets $Q \subset S$. If we let the $y_Q$ entry correspond to the set $Q$ then we have:

\begin{equation}
    y_Q = \frac{1}{N}\sum_{x'\in X} f(x_Q, x'_{\neg Q}),~~~~\text{where}~N = |X|. 
    \label{eq:kshap_regression_approximation}
\end{equation}
which is an approximation for Eq.\ref{eq:example_delta_shapley} and where we use $\neg Q$

\paragraph{Approximation 2.:} The [soundness] of this approximation relies on the assumptions of: (1) feature independence, and (2) model linearity (See Equations 11 and 12 respectively from \cite{Lundberg_Lee_2017}).


Equations \ref{eq:kshap_regression} and \ref{eq:kshap_regression_approximation} are part of the kernel-SHAP procedure \cite{Lundberg_Lee_2017}. They can both become computational bottlenecks: Eq. \ref{eq:kshap_regression} relies on $X$ that has an exponential dependence on the number of features, and Eq.\ref{eq:kshap_regression_approximation} needs $N$ model evaluations for all of the $2^M$ elements of the powerset.

\paragraph{Approximation 3.:} approximations might be needed in certain cases such as reducing the size of the dataset used (through the kMeans clustering algorithm, for example) and by reducing the number of features considered through regularisation methods such as $l_1$-norm regularisation.

==> sections/temporary_rp.tex <==
\section{Different Views on the Same Problem}

In this section, we analyse the approaches followed by existing methods for building local surrogates in the post-hoc model-agnostic setting.
We show their common construction process and make apparent the similarities and discrepancies between them.
Our focus is set in particular on how each approach tackles the notion of \emph{locality}, identifying which parts of the feature space are relevant for the instance to be explained. The notion of locality is pivotal for local surrogates and, as we will show, differences in its definition have important consequences for the explanation provided.


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/neighbourhoods}
    \caption{Neighbourhoods associated with the instances' weights (when applicable) generated by various local interpretable surrogate approaches. Setup: \textit{Half-Moons} dataset (red and blue points: 2 classes), neural network black-box represented by its decision boundary (red and blue areas). The instance of the prediction to explain (red star) is shared across the approaches. Points of the neighbourhoods are represented either with blue dots (no weights associated) or dots colored to represent the weight's value (darker equals more important weight). The neighborhoods generated, and thus the information captured to fit the surrogate, are very different while the setup and the prediction to explain are the same. }%
    \label{fig:sota_neighbourhoods}%
\end{figure}

% \footnote{For reference and comparison the detailed procedure for each approach is in appendix.}
We now review state-of-the-art approaches for building local surrogates. To illustrate the discrepancies between local surrogates, the neighbourhoods generated by every approach for the same prediction on the Half-Moons dataset are shown in Figure~\ref{fig:sota_neighbourhoods}.

\paragraph{Local Interpretable Model-Agnostic Explanations}
Arguably one of the most well-known model-agnostic local surrogate approaches is \emph{LIME}~\cite{ribeiro2016should}.
In LIME, locality is introduced in two ways, (1) by sampling instances from a Gaussian distribution centered on $\bm{z}_e$, and (2) by adding weights proportional to the exponentiated negative euclidean distance between these instances and~$\bm{z}_e$. The bandwidth(/kernel width) is based on a global heuristic depending on the dimension of the input space, hence failing to adapt to every unique case and its possible intricacies. The consequence of defining locality this way is the risk of LIME being unable to properly capture the relevant local classification behaviour of the black-box to explain a prediction~\cite{laugel2018b}. In such situations, its behaviour has been shown to be closer to the one of a global surrogate, approximating the whole black-box.


The last point combined with the simplicity and rigidness of the Gaussian distribution raises the question of .... .

An illustration of a neighbourhood generated by LIME on half-moons dataset is shown Figure~\ref{fig:lime_neigh}.

\begin{align}
    \boldsymbol{N}_{x_e}^{Lime} &= \{z_i \sim \mathcal{N}(x_e, \sigma_{Lime}) \}_{i=1}^{s_{x_e}^{Lime}} \label{eq:lime_neigh}\\
    \boldsymbol{w}_{x_e}^{Lime} &= \{w_i = \exp{\big(-\frac{1}{\gamma}\cdot \|z_i - x_e\|^2\big)} \}_{i=1}^{s_{x_e}^{Lime}} \label{eq:lime_weights}
\end{align}
where $\sigma_{Lime}$, $\gamma$ and $s_{x_e}^{Lime}$ are to be chosen.\footnote{From the implementation of LIME (https://github.com/marcotcr/lime), these values default to: scale of the data, $(\sqrt{\textit{\#features}})^{0.75}$ and $5000$, respectively.}\addtocounter{footnotecounter}{1} The weighted neighborhood is then used to train a linear decision model. LIME does not explore the decision boundary directly, but instead samples the dataset, such that it is close (in Euclidean distance) from the instance in question. 

\begin{figure}[h]
    \centering
    \includegraphics[width=7.5cm]{figures/neighs/moons/lime.pdf}
    \caption{Neighbourhood and weights from LIME.}
    \label{fig:lime_neigh}
\end{figure}

To generate local explanations for individual predictions, LIME relies on a global neighborhood generated by adding a normal perturbation to some input dataset given by the user. To bring some locality to the explanations, these instances are weighted depending on their distance to the instance whose prediction is to be interpreted.


Although these weights do bring some locality to the explanations built by LIME, the generated neighborhood is thus global.


\paragraph{Decision boundary-focused surrogates}
% LIME's sampling has been criticized by several works~\cite{laugel2018b, guidotti2018, renard2018} as being global, which highlight some locality issues created by this approach and insisted on the need to have a local neighborhood. Those propose new neighbourhood generation techniques that focus on the local decision boundary of the classifier.

% \emph{LS}~\cite{laugel2018b} is based on detecting the $l_2$-closest touch-point $CF(z_e)$ of the decision boundary and generating instances uniformly in its ($CF(z_e)$) vicinity.
To circumvent LIME's issues, \emph{LS}~\cite{laugel2018b} proposes to exploit the structure of the decision boundary and use the information provided by the nearest point of the opposite class, generating instances uniformly within a hyper-ball in its vicinity. As opposed to LIME, LS clearly defines which part of the decision boundary is relevant: the nearest point on the decision boundary.
An issue is to define how large the hyper-ball neighbourhoods should be. Furthermore, the decision boundary may require more than one touch-point in several directions to be fully captured by the neighbourhood.

The instance $CF(z_e)$ is found using the \textit{Growing Spheres} algorithm introduced in~\cite{laugel2018a}.

An illustration of a neighbourhood generated by \emph{LS} on half-moons dataset is shown Figure~\ref{fig:gsls_neigh}.



\begin{align*}
  \boldsymbol{N}_{x_e}^{LS} &= \{z_i \sim \mathcal{U}(B^{d}(CF(x_e))\}_{i=1}^{s^{LS}} \\
\end{align*}
where $B^{d}(CF(x_e))=\{x \in \mathbb{R}^{d} :\|x - CF(x_e)\|_2 \leq r \}$, where $r$ is to be chosen by the user. No weights are used.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=7.5cm]{figures/neighs/moons/gsls.pdf}
%     \caption{Neighbourhood generated using LS.}
%     \label{fig:gsls_neigh}
% \end{figure}

In \emph{Local Rule-Based Explanations} (LORE)~\cite{guidotti2018}, the authors make use of the decision boundary surrounding the instance to be explained to construct the neighbourhood.
The construction of the neighbourhood is posed as a set of optimisation problems; one for finding instances of the same class as $\bm{z}_e$, and one for finding instances not belonging to that class. The authors propose a genetic algorithm to maximise the objective functions. This allows them to detect the variations of the local decision boundary. In comparison with LS, LORE goes a step further and aims at an in-depth exploration of the decision boundary surrounding the instance.
% \todo[inline]{ISSUE ON THIS NEIGHBOURHOOD}
While they also make use of the decision boundary, and explore beyond the nearest point, there is not a clear understanding of what ``local'' means in this case.
Surrogate models can then be trained on the generated neighborhood to generate the explanations. 

An illustration of a neighbourhood generated by \emph{LORE} on half-moons dataset is shown Figure~\ref{fig:lore_neigh}.



In \emph{Local Rule-Based Explanations} (LORE)~\cite{guidotti2018}, the authors make use of the decision boundary surrounding the instance to be explained to construct the neighbourhood. The construction of the neighbourhood is posed as a set of optimization problems; one for finding instances of the same class as $\boldsymbol{x}_e$:
\begin{equation*}
    \text {fitness}_{=}^{x_e}(z)=I_{f(x_e)=f(z)}+(1-d(x_e, z))-I_{x_e=z}
\end{equation*}
and one finding instances not belonging to that class:
\begin{equation*}
    \text {fitness}_{ \neq}^{x_e}(z)=I_{f(x_e) \neq f(z)}+(1-d(x_e, z))-I_{x_e=z}
\end{equation*}
where $f$ denotes the black-box classifier, $I$ the indicator function and $d(\cdot, \cdot)$ a distance function. For the distance function the authors propose a mixture of euclidean distance, for continuous features, and simple feature matching, for discrete features. The authors propose a genetic algorithm to maximize the objective functions. This allows them to detect the variations of the local decision boundary. The size of the neighbourhood is to be chosen, with the distinct sets having equal size. Surrogate models can then be trained on the generated neighborhood to generate the explanations. 

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=7.5cm]{figures/neighs/moons/lore.pdf}
%     \caption{Neighbourhood from LORE.}
%     \label{fig:lore_neigh}
% \end{figure}

% Similarly, LAD \cite{renard2018} brings locality by generating instances globally and mapping them on the classifier's decision boundary to train a decision tree. 

\paragraph{Feature importance-based neighborhoods}
A different direction in defining the neighbourhood is based on relying on the training instances to favour the most important features. 

\emph{Local Embedding Aided Perturbation} (LEAP) \cite{localembeddings} tries to extract the relevant subspace for the instance by employing dimensionality reduction techniques at a local level. They use the \textit{Local Intrinsic Dimensionality} (LID) \cite{localembeddings} to identify the dimensionality of the subspace at the vicinity of the instance. Once the $LID$ is identified, a dimensionality reduction technique is used (e.g., Principal Components Analysis (PCA)). $\bm{z}_e$ is then projected in the new subspace giving $\hat{z}_e$. The neighbourhood and associated weights are then respectively sampled and computed similarly to LIME. The elements of the neighbourhood are then mapped back to the original feature space, where the surrogate is fitted.
% \emph{LEAP} first tries to identify the local manifold; then it proceeds in a similar fashion to \emph{LIME}, but in this sub-space of reduced dimension.
% \todo[inline]{ISSUE ON THIS NEIGHBOURHOOD}

% An illustration of a neighbourhood generated by \emph{LEAP} on half-moons dataset is shown Figure~\ref{fig:leap_neigh}.



% \emph{Local Embedding Aided Perturbation} (LEAP) \cite{localembeddings}  tries to extract the relevant subspace for the instance by employing dimensionality reduction techniques at a local level. They use the \textit{Local Intrinsic Dimensionality} (LID) to identify the dimension of the subspace at the vicinity of the instance:
% \begin{equation*}
%     \operatorname{LID}(x_e, \operatorname{Nei}(x_e))=-\left(\frac{1}{k-1} \sum_{j=1}^{k-1} \log \frac{r_{j}(x)}{r_{k}(x)}\right)^{-1}
% \end{equation*}
% where $r_{j}(x_e)$ refers to the $j^{th}$ neighbour of $x_e$ and $\operatorname{Nei}(x_e)$ to the set of $k$ nearest neighbours of $x_e$. Once the $LID$ is identified, a dimensionality reduction technique is used (e.g. Principal Components Analysis (PCA)). $x_e$ is then projected in the new subspace giving $\hat{x}_e$. The neighbourhood and associated weights are then sampled and computed (respectively) similarly to LIME (Eqs. \ref{eq:lime_neigh} and \ref{eq:lime_weights}).
% \begin{align*}
%     \boldsymbol{N}_{\hat{x}_e}^{Leap} &= \{z_i \sim \mathcal{N}(\hat{x}_e, \sigma_{Leap}) \}_{i=1}^{s_{\hat{x}_e}^{Leap}} \\
%     \boldsymbol{w}_{x_e}^{Leap} &= \{w_i = \exp{\big(- \|z_i - x_e\|^2\big)} \}_{i=1}^{s_{x_e}^{Leap}}
% \end{align*}
% The elements of $\boldsymbol{N}_{\hat{x}_e}^{Leap}$ are then mapped back to the original feature space, where the surrogate is fitted.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=7.5cm]{figures/neighs/moons/leap.pdf}
%     \caption{Neighbourhood and weights from LEAP.}
%     \label{fig:leap_neigh}
% \end{figure}

An alternative strategy is used by \emph{KernelSHAP}~\cite{lundberg2017unified}, which uses projections of the training dataset on the combinations of coordinate axes of the instance whose prediction is to be interpreted. Given $\bm{z}_e$ and the training set $\boldsymbol{X} \in \mathbb{R}^{n\times d}$, the algorithm creates altered versions of $\bm{z}_e$. To do so, it iterates over (non-empty) subsets $S$ of the $d$ features.
% iterates over all $n$ instances, then iterates over all possible (non-empty) subsets $S$ of the $d$ features.
For each subset $S$, a new instance $\bm{v}$ for the neighbourhood is generated where $\bm{v}_S = z_S$ and $\bm{v}_{\backslash S} = b_{\backslash S}$ where $b$ is an instance drawn from $\boldsymbol{X}$.
The new instance $\bm{v}$ in the neighbourhood is associated with a weight $w = \frac{d - 1}{\binom{d}{|S|} \cdot |S| \cdot (d - |S|)}$.
KernelSHAP proposes an alternative view on locality, that of exact-match based similarity measure.
To that end, it uses global information (the data) to generate the neighbourhood.
Weights also follow this direction.
KernelSHAP has the benefit that under certain assumptions you know what you are getting out: the Shapley Values \cite{shapley1952value}.
On the downside, the assumptions are very strict: 1) feature independence, and 2) (black-box) model linearity (see equations (11) and (12) respectively from \cite{lundberg2017unified}).
% \todo[inline]{ISSUE ON THIS NEIGHBOURHOOD}

% An illustration of a neighbourhood generated by \emph{KernelSHAP} on half-moons dataset is shown Figure~\ref{fig:kernelshap_neigh}.



For a given instance $v$ and a subset $S$, a new instance for the neighbourhood would be: $z$, where $z_S = x_S$ and $z_{\backslash S} = v_{\backslash S}$ with accompanying weight $w = \frac{d - 1}{\binom{d}{|S|} \cdot |S| \cdot (d - |S|)}$. 

The generating process of the neighbourhood is described below in Algo. \ref{algo:kernelshap}.

% \begin{algorithm}[tb]
%   \caption{Bubble Sort}
%   \label{alg:example}
% \begin{algorithmic}
%   \STATE {\bfseries Input:} data $x_i$, size $m$
%   \REPEAT
%   \STATE Initialize $noChange = true$.
%   \FOR{$i=1$ {\bfseries to} $m-1$}
%   \IF{$x_i > x_{i+1}$}
%   \STATE Swap $x_i$ and $x_{i+1}$
%   \STATE $noChange = false$
%   \ENDIF
%   \ENDFOR
%   \UNTIL{$noChange$ is $true$}
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[tb]
    \caption{KernelShap: Neighbourhood generating process.}
    \label{algo:kernelshap}
\begin{algorithmic}
    \STATE $\boldsymbol{N}_{x_e}^{KS} = \{ \}$
    \FOR{$\boldsymbol{z} \hspace{1mm} in \hspace{1mm} \boldsymbol{X}$}
    \STATE $\boldsymbol{x}^{tmp} = COPY(\boldsymbol{z})$
    \ENDFOR
    \FOR{subset $\boldsymbol{S} \subset [d]$}
    \STATE $\boldsymbol{x}^{tmp}_{\boldsymbol{S}} = x_{e, \boldsymbol{S}}$
    \STATE $\boldsymbol{N}_{x_e}^{KS} \leftarrow \boldsymbol{N}_{x_e}^{KS} \cup\boldsymbol{x}^{tmp}$
    \ENDFOR
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
    \caption{KernelShap: Neighbourhood generating process.}
    \label{algo:kernelshap}
     %\KwData{this text}
     %\KwResult{how to write algorithm with \LaTeX2e }
     $\boldsymbol{N}_{x_e}^{KS} = \{ \}$ \\
     \For{$\boldsymbol{z} \hspace{1mm} in \hspace{1mm} \boldsymbol{X}$}{
      $\boldsymbol{x}^{tmp} = COPY(\boldsymbol{z}$)\\
        \For{subset $\boldsymbol{S} \subset [d]$}{
            $\boldsymbol{x}^{tmp}_{\boldsymbol{S}} = x_{e, \boldsymbol{S}}$\\
            $\boldsymbol{N}_{x_e}^{KS} \leftarrow \boldsymbol{N}_{x_e}^{KS} \cup \boldsymbol{x}^{tmp}$\\
        }}
\end{algorithm}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=7.5cm]{figures/neighs/moons/kernelshap.pdf}
%     \caption{Neighbourhood and weights from KernelSHAP.}
%     \label{fig:kernelshap_neigh}
% \end{figure}

In a similar fashion to KernelSHAP, PALEX~\cite{jia2019improving} instead of constructing the full neighbourhood, as detailed in the previous paragraph, it samples from it, by randomly selecting a subset of features from $\bm{z}_e$ and replacing them with values from $\bm{X}$ (PALEX considers the empty subset as well).
A second difference comes from how weights are assigned.
The calculation of the weights relies on a set of frequent patterns extracted from the training set.
Using this set, a distance function is computed that depends on how often the two instances appear together on frequent patterns. PALEX has a similar view on locality than KernelSHAP, with the first difference lying on the fact that instead of complete enumeration of the dataset, it samples from it.
A second difference is the weight function that utilises pattern mining.
This type of weighting function goes beyond the euclidean measure and aims at identifying manifolds in the global data structure.
% \todo[inline]{ISSUE ON THIS NEIGHBOURHOOD}

An illustration of a neighbourhood generated by \emph{PALEX} on half-moons dataset is shown Figure~\ref{fig:palex_neigh}.

\begin{equation*}
    \operatorname{d}(x, z | P S)=\sum_{i=1}^M\left|\phi_i(x)-\phi_i(z)\right|
\end{equation*}

\begin{equation*}
    \phi_i(x))=\left\{\begin{array}{ll}{\operatorname{supp}\left(p_{i}\right),} & {x \text { matches } p_{i}} \\ {0,} & {\text { otherwise }}\end{array}\right.
\end{equation*}
where $PS=\left\{p_{1}, p_{2}, \ldots, p_{M}\right\}$ denotes the set of $M$ frequent patterns, mined from the data ($\boldsymbol{X}$).

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=7.5cm]{figures/neighs/moons/palex.pdf}
%     \caption{Neighbourhood and weights from PALEX.}
%     \label{fig:palex_neigh}
% \end{figure}

%The purpose of a local surrogate is to understand how the black-box is behaving in the vicinity of the instance in question.

\paragraph{Comparison} We will refer to the instance to be explained as the `subject' for brevity. The approaches we just described follow the \textit{Local Surrogate Procedure} \footnote{Even though in some of the papers we discussed, the two are mixed together, we differentiate them here, and treat them as separate components. We do appreciate though that in the case of KernelSHAP under certain assumptions on the black-box, and certain modelling choices you can get guarantees on the outputs.}. \emph{LIME} made the first step by introducing locality using targeted sampling, through a Gaussian distribution centered on the subject, and by adding complementary weights derived from closeness in Euclidean distance. The standard deviation is based on a global heuristic that does not adapt to every case and its intricacies. The last point combined with the simplicity and rigidness of the Gaussian distribution raises the question of .... . \emph{LS} proposes to exploit the structure of the decision boundary, and exploit the information of the nearest point of the opposite class. As opposed to \emph{LIME}, \emph{LS} has a clear view of which part of the decision boundary is relevant: the nearest point on the decision boundary, and a ball around it. The issue here, is how large of a ball to consider? \emph{LORE} goes a step further and aims at an in-depth exploration of the decision boundary surrounding the instance. While they also make use of the decision boundary, and explore beyond the nearest point, there is not a clear understanding of what ``local'' means in this case. \emph{KernelSHAP} proposes an alternative view on locality, that of exact-match based similarity measure. To that end, it uses global information (the data) to generate the neighbourhood. Weights also follow in this direction. \emph{KernelSHAP} has the benefit that under certain assumptions you know what you are getting out: the Shapley Values. On the downside, the assumptions are very strict: 1) feature independence, and 2) (black-box) model linearity (see equations (11) and (12) respectively from \cite{lundberg2017unified}).


\emph{PALEX} has a similar view on locality, with the first difference lying on the fact that instead of complete enumeration of the dataset, \emph{it samples from it}. A second difference is the weight function that utilises pattern mining. This type of weighting function goes beyond the euclidean measure and aims at identifying manifolds in the global data structure. 

\emph{LEAP} is different takes a step in a different direction as it first tries to identify the local manifold; then it proceeds in a similar fashion to LIME, but in this sub-space of reduced dimension.

\todo[inline]{improve the big picture of the issues of neighbourhoods with current local surrogates / explanations not traceable with an objective}

% \subsection{Locality is the main pitfall to formalise local surrogates}
\subsection{When should I trust you? The pitfall of locality}

While all these approaches might lead to seemingly adequate surrogates and provide added value to the practitioner, there is a lack of consensus on properties these models should possess. There is a general agreement that the surrogate should reflect the behaviour of the black-box in the locality of the instance to be explained, but beyond this not much. The crux of local surrogates is on identifying what \emph{locality} really means, and then modelling it through the means of fitting an interpretable surrogate on the generated neighbourhood.

Furthermore, there is no consensus as to what is the objective of \emph{Local Surrogates}. \emph{\textbf{The output cannot be traced back to an objective}}. There is no real understanding of what the output means, because there is not a well-defined objective. This is what we tackle in the following section.

% From previous paper; might be useful
% A second point, that we elaborate on further in the following section, is the lack of explicit consideration, or even (we believe) wrong view of explanation smoothness\footnote{With explanation smoothness we imply the robustness of the explanation provided to small perturbations in the input. See Eq. \ref{eq:explanation_smoothness} in the following section.}. Our approach aims at uncovering the relevant decision boundary and using it to construct the neighbourhood. While relevant can be defined in many ways we view it through \textit{feature invariances}, and aim at constructing neighbourhoods by putting together instances that share the same invariances. As will be discussed in the following section, our goal with this scheme is for instances that share the same relevant decision boundary (or have similar invariances) to have the same explanations as well.

% Table~\ref{tab:background} illustrates our categorization of the presented approaches.

% \begin{table}[h]
%     \centering
%     \begin{tabular}{c|c|c|c|c}
%     approach & locality & meaningful & surrogate & nh size  \\
%     \hline
%     LIME & glob+w &  No & imposed & user \\
%     LS & local &  No & imposed & user\\
%     KernelSHAP & local & for the train & imposed & imposed\\
%     LAD & local & No & imposed & user \\
%     LORE & local & No & imposed & user \\
%     LEAP & local & for the train & free & user \\
%     PALEX & local & for the train & free & user \\
%     \hline
% \end{tabular}
%     \caption{1) If table is kept, update columns. 2)If we propose our own approach to minimize invariacne, then add it to show it is the only one that does XXX.}
%     \label{tab:background}
% \end{table}

% \begin{table}[h]
%     \centering
%     \begin{tabular}{c|c|c|c}
%     approach & locality &  nh size & relevance  \\
%     \hline
%     LIME & glob+w & user & decision boundary \\
%     LS & local & user & closest touchpoint \\
%     KernelSHAP & local & imposed & train\\
%     LAD & local & user & decision boundary \\
%     LORE & local & user & decision boundary \\
%     LEAP & local & user & train \\
%     PALEX & local & user & train \\
%     \textbf{Our proposition} & \textbf{local} & \textbf{imposed} & \textbf{decision boundary} \\
%     \hline
% \end{tabular}
%     \caption{Proposition2}
%     \label{tab:background}
% \end{table}



% \includegraphics[width=5cm]{figures/neighs/moons/lime.pdf}
% \includegraphics[width=5cm]{figures/neighs/moons/gsls.pdf}
% \includegraphics[width=5cm]{figures/neighs/moons/kernelshap.pdf}
% \includegraphics[width=5cm]{figures/neighs/moons/leap.pdf}
% \includegraphics[width=5cm]{figures/neighs/moons/lore.pdf}
% \includegraphics[width=5cm]{figures/neighs/moons/palex.pdf}
